Triamese-ViT: A 3D-Aware Method for Robust Brain Age Estimation from MRIs

The integration of machine learning in medicine has significantly improved diagnostic precision, particularly in the interpretation of complex structures like the human brain. Diagnosing challenging conditions such as Alzheimer's disease has prompted the development of brain age estimation techniques. These methods often leverage three-dimensional Magnetic Resonance Imaging (MRI) scans, with recent studies emphasizing the efficacy of 3D convolutional neural networks (CNNs) like 3D ResNet. However, the untapped potential of Vision Transformers (ViTs), known for their accuracy and interpretability, persists in this domain due to limitations in their 3D versions. This paper introduces Triamese-ViT, an innovative adaptation of the ViT model for brain age estimation. Our model uniquely combines ViTs from three different orientations to capture 3D information, significantly enhancing accuracy and interpretability. Tested on a dataset of 1351 MRI scans, Triamese-ViT achieves a Mean Absolute Error (MAE) of 3.84, a 0.9 Spearman correlation coefficient with chronological age, and a -0.29 Spearman correlation coefficient between the brain age gap (BAG) and chronological age, significantly better than previous methods for brian age estimation. A key innovation of Triamese-ViT is its capacity to generate a comprehensive 3D-like attention map, synthesized from 2D attention maps of each orientation-specific ViT. This feature is particularly beneficial for in-depth brain age analysis and disease diagnosis, offering deeper insights into brain health and the mechanisms of age-related neural changes.

==> sec/copy.tex <==
In this section, we will introduce the structure of Triamese-ViT. As we show in Figure \ref{figure 2}, the idea of Triamese-ViT is inspired by ~\cite{dosovitskiy2020image} and ~\cite{gupta2023siamese}. The input of Triamese-ViT are 3D MRIs, we called the images $I$$\in$$R^{H\times W\times C}$, here H, W, C are image height, width and number of channels. Then we reshape the image $I$ into 3 different viewpoints, $I$$\to$($I_x$,$I_y$,$I_z$), $I_x$$\in$$R^{H\times W\times C}$,$I_y$$\in$$R^{H\times C\times W}$,$I_z$$\in$$R^{W\times H\times C}$.
Firstly, we focus on $I_x$, we change it to a sequence of flattened 2D patches called $I_{x,p}$$\in$$R^{N\times(p^{2}\cdot C)}$, the patches are squares of length $P$. So the number of patches is $N=H\times W/P^{2}$.
In all of the layers in the transformer encoder, vectors with dimension D will be processed as the object, so we need to map $I_x$ to D dimensions with a trainable linear projection. The formulate is shown below:
\begin{equation}
z_{x,0}=Concat(I_{x,class};I_{x,p}^{1}E;I_{x,p}^{2}E;...;I_{x,p}^{N}E)+E_{pos}
\label{1}
\end{equation}
In Eq. \ref{1}, $I_{x,class}$ means a learnable token, in other words, the class token, which is added into ViT, this method is similar to ~\cite{devlin2018bert}. Note that $I_{x,class}$ will finally output from the Transformer Encoder as $z_{x,L}^{0}$, which represents the image representation $P$ (Eq. \ref{7}). $E \in R^{(p^{2}\cdot C)\times D}$ means Linear Projection, $Concat$ means token concatenation and $E_{pos} \in R^{(N+1)\times D}$ represents positional information which is added to each token embedding. We use the same pre-processing methods on $I_y$ and $I_z$, and we can get $z_{y,0}$ and $z_{z,0}$.

Now, the original data is processed into three suitable matrices $z_{x,0},z_{y,0},z_{z,0} \in R^{(N+1)\times D}$, then we feed them to the transformer encoder. Each Transformer encoder is a multi-layered system where the input sequentially passes through several key components in each layer: it first encounters a Layer Normalization (LN), followed by a Multi-Head Attention mechanism, another Layer Normalization, and then a Multi-Layer Perceptron (MLP). The Multi-Head Attention (MSA) operates by conducting parallel attention calculations across multiple 'heads', diversifying the focus and allowing for a richer understanding of the input data.
\begin{equation}
[Q,K,V]=FC(z_{x,0})
\label{2}
\end{equation}
Here, $Q\in R^{(N+1)\times d}$,$K\in R^{(N+1)\times d}$,$V\in R^{(N+1)\times d}$ represent Query, Keyword and Value. We assume the number of heads in MSA is n, and $D=n\times d$. Each 'head' independently processes the input, allowing the model to simultaneously attend to information from different representation subspaces at different positions.
\begin{equation}
head_{i}=softmax(\frac{Q_{i}K_{i}^{\mathsf{T}}}{\sqrt{d}}V_{i})
\label{3}
\end{equation}
\begin{equation}
MSA(z_{x,0})=Concat(head_{1},head_{2},...,head_{n})
\label{4}
\end{equation}

Let $z_{x,0}$ be the input of the first layer Transformer Encoder, so the feedforward calculation in the Encoder is written as:
\begin{equation}
z_{x,l}^{'}=MSA(LN(z_{x,l-1}))+z_{x,l-1}
\label{5}
\end{equation}
\begin{equation}
z_{x,l}=MLP(LN(z_{x,l}^{'}))+z_{x,l}^{'}
\label{6}
\end{equation}
The $l\in [1,2,...L]$. The outputs from each Transformer Encoder are channeled into an MLP (Multi-Layer Perceptron) head, comprising a hidden layer followed by an output layer, to generate the final prediction for each view. We denote the prediction from the $I_{x}$ (the first view) as $P_{x}$. Applying the same procedure to the $I_{y}$ and $I_{z}$ views, we obtain two additional predictions, $P_{y}$ and $P_{z}$, corresponding to these orientations.

In the final stage, these three view-based predictions ($P_{x}$, $P_{y}$, and $P_{z}$) are input into the Triamese MLP. This step integrates the insights from all three views to produce the model's comprehensive final prediction.
\begin{equation}
P= MLP(P_{x},P_{y},P_{z})
\label{7}
\end{equation}

We experimented with various strategies to integrate the outputs from the three viewpoint-specific ViTs. These strategies included averaging the results, selecting the best-performing output, and combining the outputs through an MLP. Our experiments demonstrated that processing the results through an MLP yielded the most effective performance. The loss function used in the training is the Mean Squared Error (MSE) between the predicted age $P_{i}$ and chronological age $C_{i}$.
\begin{equation}
Loss=\frac{\sum_{i=1}^{n}(P_{i}-C_{i})^{2}}{n}
\label{8}
\end{equation}




The integration of machine learning in medicine has notably enhanced diagnostic precision, particularly in interpreting complex structures like the human brain. Diagnosing brain conditions such as Alzheimer’s disease remains challenging, prompting the development of brain age estimation techniques. These techniques often utilize three-dimensional Magnetic Resonance Imaging (MRI) scans, with recent studies highlighting the efficacy of 3D convolutional neural networks (CNNs) like 3D ResNet. However, the potential of Vision Transformers (ViTs) in this domain, especially known for their accuracy and interpretability, has not been fully tapped due to the limitations of their 3D versions. In response, this paper introduces Triamese-ViT, an innovative adaptation of the ViT model, used for for brain age estimation. Our model uniquely combines ViTs from three different orientations, leading to significantly enhanced accuracy and interpretability. Tested on a dataset of 1351 MRI scans, Triamese-ViT achieves a Mean Absolute Error (MAE) of 3.84, a 0.9 Spearman correlation coefficient with chronological age, and a -0.29 Spearman correlation coefficient between the brain age gap (BAG) and chronological age. A key innovation of Triamese-ViT is its ability to produce a comprehensive 3D-like attention map, synthesized from 2D attention maps of each orientation-specific ViT. This feature is particularly beneficial for in-depth brain age analysis and disease diagnosis, providing deeper insights into brain health and the mechanisms of age-related neural changes.


Aging is a natural part of life, and as we grow older, every part of our body begins to show the effects of time, including our brain. The brain is incredibly sensitive and undergoes complex changes that increase the risk of diseases like Alzheimer's as we age. Unfortunately, traditional methods for diagnosing brain diseases can be slow and unreliable, often depending too much on a doctor’s judgment~\cite{avants2008symmetric,liu2015low}. This can lead to delayed or incorrect diagnoses, which may cost valuable treatment time and potentially worsen the patient’s condition.

Thanks to advances in artificial intelligence, doctors are turning to machine learning for better and faster brain diagnoses~\cite{cole2017predicting,feng2020estimating,armanious2021age,zhang2022robust}. A great example of this is the brain age estimation project. This approach uses machine learning or deep learning to analyze brain images and estimate how old the brain looks. The trained model which has learned the age-specific pattern of healthy people's brains, will extract the patient's brain features and predict the age of the brain in this status. This estimated brain age is then compared to the patient's actual age. If the prediction is less than chronological age, it represents the patient's brain is activated and healthy, on the contrary,  shows some diseases influence the patient's brain~\cite{cole2017predicting,beheshti2018association,gaser2013brainage}. 

The difference between the estimated brain age and the patient's actual age is known as the brain age gap (BAG). Several researches have proved that it has a great relation to age-related brain diseases such as AD~\cite{beheshti2018association}, psychosis~\cite{chung2018use}, mild cognitive impairment (MCI)~\cite{gaser2013brainage}, major depressive disorder~\cite{han2021brain}, mortality~\cite{cole2018brain}, and others~\cite{kaufmann2019common}. Since many brain diseases still lack effective treatments, improving algorithms for estimating brain age is crucial. It can help us catch these diseases early, offering hope to patients who are still in search of relief.

Most of the current methods for estimating brain age rely on convolutional neural networks (CNNs), which are trained on either 3D MRI scans or 2D slices taken from these scans.~\cite{cole2017predicting,huang2017age,hong2020brain,bellantuono2021predicting} CNNs are incredibly adept at handling image-related tasks; they can take in the entire set of data from 3D MRIs to offer a well-rounded prediction. However, CNNs typically focus on the most noticeable features across the entire image, which often leads to a neglect of finer details—details that are crucial for accurate predictions~\cite{alzubaidi2021review}, particularly when it comes to the complexities of the brain. Additionally, a significant hurdle with CNNs lies in their lack of transparency. They do not easily reveal the rationale behind their predictions, a stumbling block when it comes to Explainable AI—an emerging field that emphasizes the importance of understanding and interpreting AI decisions. This opacity becomes a challenge in medical diagnostics, as it hampers the ability to pinpoint the exact location of brain abnormalities or diseases when using CNN-based models.

Compared to traditional CNN models, the Vision Transformer (ViT) offers a unique advantage when it comes to focusing on image details~\cite{dosovitskiy2020image}. It does this by breaking down the image into smaller pieces, known as patches. These patches are then processed using a convolutional layer that transforms each one into a high-dimensional space, allowing the model to extract detailed information and understand how different parts of the image interact with each other~\cite{khan2022transformers}. What makes ViT stand out is its ability to show us how it focuses on the image through something called an attention map, which helps us see why it makes certain predictions. Despite these strengths, ViT isn't perfect. It sometimes misses out on the bigger picture because it doesn't always capture the global context well. Another issue is that ViT is mostly used for 2D images. This can be a problem for brain age prediction because it means researchers often use flat 2D slices of MRI scans as input~\cite{he2021global}. Although this approach can greatly reduce the time of training and prediction, it doesn't take into account the full 3D structure of the brain, leading to a loss of important depth information.

To address the need for both detailed analysis and understanding of interactions across different areas within an image, we introduce a new model, Triamese-ViT. This model is inspired by the Siamese Masked Autoencoders concept developed by Agrim Gupta and his colleagues~\cite{gupta2023siamese}. The novelty of this model is that it adeptly transforms 3D imaging challenges into a 2D analytical framework, effectively preserving the rich information contained in three-dimensional images, and has the same fast process speed as 2D images at the same time. A standout feature of our model is its capability to generate 3D-like attention maps, offering profound interpretability. These maps have been meticulously compared with conventional Explainable AI (XAI) methods and corroborated with findings from relevant medical research~\cite{shine2023impact,smajic2022single,russo2022age,xiong2022altered,wang2022roles}, affirming their scientific validity, logical coherence, and precision. This synergy of advanced imaging analysis and interpretability positions our model as a significant tool in medical diagnostics and research, especially in areas demanding high fidelity in three-dimensional medical data understanding. We trained and tested our model on MRI scans from 1351 healthy individuals. When compared with the state-of-the-art algorithms, Triamese-ViT not only showed superior predictive accuracy but also demonstrated improvements in fairness and interoperability. Our model achieves impressive results that mean absolute error (MAE) of 3.87, a 0.93 Spearman correlation coefficient when comparing predicted brain age to chronological age, and a -0.29 Spearman correlation coefficient between the chronological age and the brain age gap (the absolute value of the gap between the predicted and actual age). In addition, we subjected our model to Explainable AI (XAI) techniques, such as 3D occlusion analysis, to validate the high-correlation areas identified by the model. These areas matched those highlighted by the attention maps produced by Triamese-ViT, reinforcing the validity of our model’s interpretive output.


This section will introduce the background of brain age estimation. Traditionally, predicting a brain's age involved extracting specific features from MRI scans, then using those features in a classification or regression model to estimate age. Yet, this approach has its drawbacks. Manually chosen features may not capture all the nuances necessary to accurately reflect brain age. In particular, image pre-processing involves a degree of subjective decision-making that necessitates various assumptions. These assumptions are rarely met in practice, potentially leading to inaccuracies in the model, as evidenced in studies~\cite{avants2008symmetric,liu2015low}. Moreover, the manual extraction of features is not only prone to potential oversight but is also time-intensive. When it comes to medical decision-making, every minute counts. The need for swift action to prevent treatment delays means that slow and laborious processes have no place in practical applications. These critical issues have significantly limited the broader adoption of brain age prediction methods in clinical settings.

The field of brain age estimation has advanced significantly with the application of convolutional neural networks (CNNs). Since 2017, CNNs have been at the forefront, favored for their ability to autonomously extract features and deliver high-accuracy results~\cite{bellantuono2021predicting,pardakhti2020brain,jiang2020predicting,hong2020brain}. Cole et al.~\cite{cole2017predicting} demonstrated this by training a 3D CNN on MRI samples, finding that models trained on gray matter outperformed those trained on white matter. To enhance efficiency, researchers have turned to 2D MRI slices, with ~\cite{lam2020accurate} using recurrent neural networks (RNN) to understand the connections between slices, offering a balance between performance and computational demand. Then, the advanced and special CNN structure such as SFCN, ResNet, and DenseNet also highlighted their strength in this area~\cite{ning2021improving,mouches2022multimodal,wood2022accurate}. When the transformer is applied in the models, since it can help pay more attention to details of the images, it is very suitable for use in the medical field. For instance, the Global–Local Transformer~\cite{he2021global} melds the strengths of CNNs with transformers, utilizing 2D MRI slices to capture both local and global information in the images. Cai et al.~\cite{cai2022graph} furthered this approach by leveraging a graph transformer network in a multimodal method, efficiently harnessing both global and local features for brain age estimation.

\subsection{Explainable AI (XAI)}
Since we will use XAI techniques to prove our model's ability to interpretability, we introduce the background of XAI in this section. AI advancements have empowered diverse data-driven applications across multiple disciplines, including but not limited to neuroscience, biology, chemistry, engineering, psychology, education, psychology, and philosophy~\cite{langer2021we,langer2021explainability,doshi2017towards,ali2023explainable}. Despite its wide-ranging utility, AI often operates as a "black box," with complex models and a multitude of parameters obscuring the decision-making process. This lack of transparency is particularly critical in sensitive fields such as finance~\cite{cao2022ai} and healthcare~\cite{caruana2015intelligible}, where understanding AI's reasoning is crucial, so this need boosts the development of XAI. 

XAI methods generally fall into two categories~\cite{longo2023explainable,das2020opportunities}: backpropagation-based and perturbation-based. Backpropagation-based XAI involves algorithms that provide insight during the backpropagation stage of neural network processing, typically by using derivatives to produce attribution maps like class activation or saliency maps. On the other hand, perturbation-based approaches modify the input features in various ways—through occlusion, substitution, or generative techniques—to observe changes in the output. Our project employs occlusion analysis, a perturbation-based technique, to validate our model's interpretability.

